Tri-Attention: Explicit Context-Aware Attention Mechanism for Natural Language Processing

In natural language processing (NLP), the context of a word or sentence plays an essential role. Contextual information such as the semantic representation of a passage or historical dialogue forms an essential part of a conversation and a precise understanding of the present phrase or sentence. However, the standard attention mechanisms typically generate weights using query and key but ignore context, forming a Bi-Attention framework, despite their great success in modeling sequence alignment. This Bi-Attention mechanism does not explicitly model the interactions between the contexts, queries and keys of target sequences, missing important contextual information and resulting in poor attention performance. Accordingly, a novel and general triple-attention (Tri-Attention) framework expands the standard Bi-Attention mechanism and explicitly interacts query, key, and context by incorporating context as the third dimension in calculating relevance scores. Four variants of Tri-Attention are generated by expanding the two-dimensional vector-based additive, dot-product, scaled dot-product, and bilinear operations in Bi-Attention to the tensor operations for Tri-Attention. Extensive experiments on three NLP tasks demonstrate that Tri-Attention outperforms about 30 state-of-the-art non-attention, standard Bi-Attention, contextual Bi-Attention approaches and pretrained neural language models1.

==> mybibfile_fullconferencename_.tex <==
@inproceedings{Zhang21,
  title = {Enlivening Redundant Heads in Multi-head Self-attention for Machine Translation},
  author = {Zhang, Tianfu and Huang, Heyan and Feng, Chong and Cao, Longbing},
  booktitle = {Proceedings of the 2021 Conference on Empirical Methods in Natural Language Processing},
  pages = {3238--3248},
  year = {2021}
}

@ARTICLE{Tensor_Kolda2009,
	AUTHOR = "T.G. Kolda and B.W. Bader",
	TITLE = "Tensor decompositions and applications",
	JOURNAL = "SIAM Review",
	VOLUME = {51},
	NUMBER = {3},
	PAGES = {455-500},
	MONTH = "",
	YEAR = {2009}
}

@inproceedings{zhang2021graph,
  title={Graph-based tri-attention network for answer ranking in {CQA}},
  author={Zhang, Wei and Chen, Zeyuan and Dong, Chao and Wang, Wen and Zha, Hongyuan and Wang, Jianyong},
  booktitle={Proceedings of the 35th AAAI Conference on Artificial Intelligence},
  pages={14463--14471},
  year={2021}
}

@inproceedings{guan2022block,
  title={Block-{S}kim: {E}fficient question answering for {T}ransformer},
  author={Guan, Yue and Li, Zhengyi and Lin, Zhouhan and Zhu, Yuhao and Leng, Jingwen and Guo, Minyi},
  booktitle={Proceedings of the 36th AAAI Conference on Artificial Intelligence},
  pages={10710--10719},
  year={2022}
}

@ARTICLE{Zhang2021LadRa,
  author={Zhang, Kun and Lv, Guangyi and Wu, Le and Chen, Enhong and Liu, Qi and Wang, Meng},
  journal={IEEE Transactions on Neural Networks and Learning Systems}, 
  title={{LadRa-Net}: {L}ocally Aware Dynamic Reread Attention Net for Sentence Semantic Matching}, 
  year={2021},
  volume={1},
  number={1},
  pages={1-14}
 }

@ARTICLE{Benjamins2022,
  author={Carolin Benjamins and Theresa Eimer and Frederik Schubert and Aditya Mohan and Andre Biedenkapp and Bodo Rosenhahn and Frank Hutter and Marius Lindauer},
  journal={ArXiv Preprint}, 
  title={Contextualize Me - {T}he Case for Context in Reinforcement Learning}, 
  year={2022},
  volume={},
  number={},
  pages={arXiv:2202.04500}
 }

@ARTICLE{Hallak2015,
  author={Assaf Hallak and Dotan Di Castro and Shie Mannor},
  journal={ArXiv Preprint}, 
  title={Contextual {M}arkov Decision Processes}, 
  year={2015},
  volume={},
  number={},
  pages={arXiv:1502.02259 }
 }

@inproceedings{Zeng2021recurrent,
  title={Recurrent attention for neural machine translation},
  author={Zeng, Jiali and Wu, Shuangzhi and Yin, Yongjing and Jiang, Yufan and Li, Mu},
  booktitle={Proceedings of the 2021 Conference on Empirical Methods in Natural Language Processing},
  pages={3216--3225},
  year={2021}
}

@inproceedings{rashed2022context,
  title={Context and Attribute-Aware Sequential Recommendation via Cross-Attention},
  author={Rashed, Ahmed and Elsayed, Shereen and Schmidt-Thieme, Lars},
  booktitle={Proceedings of the 16th ACM Conference on Recommender Systems},
  pages={71--80},
  year={2022}
}

@inproceedings{pang2022heterogeneous,
  title={Heterogeneous global graph neural networks for personalized session-based recommendation},
  author={Pang, Yitong and Wu, Lingfei and Shen, Qi and Zhang, Yiming and Wei, Zhihua and Xu, Fangli and Chang, Ethan and Long, Bo and Pei, Jian},
  booktitle={Proceedings of the 15th ACM International Conference on Web Search and Data Mining},
  pages={775--783},
  year={2022}
}

@inproceedings{zheng2022family,
  title={A Family of Neural Contextual Matrix Factorization Models for Context-Aware Recommendations},
  author={Zheng, Yong and Florez Arias, Gonzalo},
  booktitle={Adjunct Proceedings of the 30th ACM Conference on User Modeling, Adaptation and Personalization},
  pages={1--6},
  year={2022}
}

@article{zhang2021neural,
  title={Neural time-aware sequential recommendation by jointly modeling preference dynamics and explicit feature couplings},
  author={Zhang, Qi and Cao, Longbing and Shi, Chongyang and Niu, Zhendong},
  journal={IEEE Transactions on Neural Networks and Learning Systems},
  year={2021}
}


@article{zhu2020unsupervised,
  title={Unsupervised heterogeneous coupling learning for categorical representation},
  author={Zhu, Chengzhang and Cao, Longbing and Yin, Jianping},
  journal={IEEE Transactions on Pattern Analysis and Machine Intelligence},
  volume={44},
  number={1},
  pages={533--549},
  year={2020}
}

@article{cao2022personalized,
  title={Personalized next-best action recommendation with multi-party interaction learning for automated decision-making},
  author={Cao, Longbing and Zhu, Chengzhang},
  journal={Plos one},
  volume={17},
  number={1},
  pages={e0263010},
  year={2022}
}

@article{cao2022beyond,
  title={Beyond {IID}: {Non-IID} thinking, informatics, and learning},
  author={Cao, Longbing},
  journal={IEEE Intelligent Systems},
  volume={37},
  number={4},
  pages={5--17},
  year={2022}
}

@inproceedings{hu2019introductory,
	title={An introductory survey on attention mechanisms in {NLP} problems},
	author={Hu, Dichao},
	booktitle={Proceedings of SAI Intelligent Systems Conference},
	pages={432--448},
	year={2019}
}

@inproceedings{wang2020decoupled,
	title={Decoupled attention network for text recognition},
	author={Wang, Tianwei and Zhu, Yuanzhi and Jin, Lianwen and Luo, Canjie and Chen, Xiaoxue and Wu, Yaqiang and Wang, Qianying and Cai, Mingxiang},
	booktitle={Proceedings of the 34th AAAI Conference on Artificial Intelligence},
	pages={12216--12224},
	year={2020}
}

@inproceedings{Vaswani2017Attention,
	author    = {Ashish Vaswani and
	Noam Shazeer and
	Niki Parmar and
	Jakob Uszkoreit and
	Llion Jones and
	Aidan N. Gomez and
	Lukasz Kaiser and
	Illia Polosukhin},
	title     = {Attention is All you Need},
	booktitle = {Proceedings of the Advances in Neural Information Processing Systems},
	pages     = {5998--6008},
	year      = {2017}
}

@article{basiri2021abcdm,
	title={ABCDM: {A}n attention-based bidirectional {CNN-RNN} deep model for sentiment analysis},
	author={Basiri, Mohammad Ehsan and Nemati, Shahla and Abdar, Moloud and Cambria, Erik and Acharya, U Rajendra},
	journal={Future Generation Computer Systems},
	volume={115},
	number={115},
	pages={279--294},
	year={2021}
}

@inproceedings{Ding2020Self,
	author    = {Liang Ding and
	Longyue Wang and
	Dacheng Tao},
	title     = {Self-attention with cross-lingual position representation},
	booktitle = {Proceedings of the 58th Annual Meeting of the Association for Computational Linguistics},
	pages     = {1679--1685},
	year      = {2020}
}

@inproceedings{Alessandro2020Fixed,
	author    = {Alessandro Raganato and
	Yves Scherrer and
	J{\"{o}}rg Tiedemann},
	title     = {Fixed encoder self-attention patterns in transformer-based machine translation},
	booktitle = {Proceedings of the 2020 Conference on Empirical Methods in Natural Language Processing},
	pages     = {556--568},
	year      = {2020}
}

@inproceedings{Ilya2019Decoupled,
	author    = {Ilya Loshchilov and
	Frank Hutter},
	title     = {Decoupled weight decay regularization},
	booktitle = {Proceedings of the 7th International Conference on Learning Representations},
	pages     = {1--18},
	year      = {2019}
}

@article{yu2021sentence,
	title={Sentence pair modeling based on semantic feature map for human interaction with IoT devices},
	author={Yu, Rui and Lu, Wenpeng and Lu, Huimin and Wang, Shoujin and Li, Fangfang and Zhang, Xu and Yu, Jiguo},
	journal={International Journal of Machine Learning and Cybernetics},
	pages={1--19},
	year={2021}
}

@inproceedings{ye2020financial,
	title={Financial risk prediction with multi-Round {Q\&A} attention network},
	author={Ye, Zhen and Qin, Yu and Xu, Wei},
	booktitle={Proceedings of the 29th International Joint Conference on Artificial Intelligence},
	pages={4576--4582},
	year={2020}
}

@inproceedings{hu2021context,
  author    = {Zhe Hu and
               Zuohui Fu and
               Yu Yin and
               Gerard de Melo},
  title     = {Context-Aware Interaction Network for Question Matching},
  booktitle = {Proceedings of the 2021 Conference on Empirical Methods in Natural Language Processing},
  pages     = {3846--3853},
  year      = {2021}
}

@article{storks2019recent,
	title={Recent advances in natural language inference: {A} Survey of benchmarks, resources, and approaches},
	author={Storks, Shane and Gao, Qiaozi and Chai, Joyce Y},
	journal={arXiv preprint arXiv:1904.01172},
	year={2019}
}

@article{Lu2021Sentence,
	author    = {Wenpeng Lu and
	Rui Yu and
	Shoujin Wang and
	Can Wang and
	Ping Jian and
	Heyan Huang},
	title     = {Sentence Semantic Matching Based on {3D CNN} for Human-Robot Language
	Interaction},
	journal   = {{ACM} Transactions on Internet Technology},
	volume    = {21},
	number    = {4},
	pages     = {98:1--98:24},
	year      = {2021}
}

@inproceedings{Yang2019Simple,
	author    = {Runqi Yang and
	Jianhai Zhang and
	Xing Gao and
	Feng Ji and
	Haiqing Chen},
	title     = {Simple and effective text matching with richer alignment features},
	booktitle = {Proceedings of the 57th Conference of the Association for Computational Linguistics},
	pages     = {4699--4709},
	year      = {2019}
}

@inproceedings{Xu2015Show,
	author    = {Kelvin Xu and
	Jimmy Ba and
	Ryan Kiros and
	Kyunghyun Cho and
	Aaron C. Courville and
	Ruslan Salakhutdinov and
	Richard S. Zemel and
	Yoshua Bengio},
	title     = {Show, attend and tell: {N}eural image caption generation with visual
	Attention},
	booktitle = {Proceedings of the 32nd International Conference on Machine Learning},
	pages     = {2048--2057},
	year      = {2015}
}

@inproceedings{Bahdanau2015Neural,
	author    = {Dzmitry Bahdanau and
	Kyunghyun Cho and
	Yoshua Bengio},
	title     = {Neural machine translation by jointly learning to align and translate},
	booktitle = {Proceedings of the 3rd International Conference on Learning Representations},
	pages     = {1--15},
	year      = {2015}
}

@inproceedings{Mnih2014Recurrent,
	author    = {Volodymyr Mnih and
	Nicolas Heess and
	Alex Graves and
	Koray Kavukcuoglu},
	title     = {Recurrent models of visual attention},
	booktitle = {Proceedings of the Advances in Neural Information Processing Systems},
	pages     = {2204--2212},
	year      = {2014}
}

@inproceedings{Ashish2017Attention,
	author    = {Ashish Vaswani and
	Noam Shazeer and
	Niki Parmar and
	Jakob Uszkoreit and
	Llion Jones and
	Aidan N. Gomez and
	Lukasz Kaiser and
	Illia Polosukhin},
	title     = {Attention is all you need},
	booktitle = {Proceedings of the Advances in Neural Information Processing Systems 30},
	pages     = {5998--6008},
	year      = {2017}
}

@inproceedings{Jacob2019BERT,
	author    = {Jacob Devlin and
	Ming{-}Wei Chang and
	Kenton Lee and
	Kristina Toutanova},
	title     = {{BERT:} {P}re-training of deep Bidirectional transformers for language
	understanding},
	booktitle = {Proceedings of the 2019 Conference of the North American Chapter of
	the Association for Computational Linguistics},
	pages     = {4171--4186},
	year      = {2019}
}

@inproceedings{Peng2020Enhanced,
	author    = {Shuang Peng and
	Hengbin Cui and
	Niantao Xie and
	Sujian Li and
	Jiaxing Zhang and
	Xiaolong Li},
	title     = {Enhanced-RCNN: {A}n efficient method for learning sentence similarity},
	booktitle = {Proceedings of The Web Conference 2020},
	pages     = {2500--2506},
	year      = {2020}
}

@inproceedings{yang2019context,
	title={Context-aware self-attention networks},
	author={Yang, Baosong and Li, Jian and Wong, Derek F and Chao, Lidia S and Wang, Xing and Tu, Zhaopeng},
	booktitle={Proceedings of the 33rd AAAI Conference on Artificial Intelligence},
	pages={387--394},
	year={2019}
}

@inproceedings{Ding2020Context,
	author    = {Liang Ding and
	Longyue Wang and
	Di Wu and
	Dacheng Tao and
	Zhaopeng Tu},
	title     = {Context-aware cross-attention for non-autoregressive translation},
	booktitle = {Proceedings of the 28th International Conference on Computational Linguistics},
	pages     = {4396--4402},
	year      = {2020}
}

@inproceedings{Luong2015Effective,
	author    = {Thang Luong and
	Hieu Pham and
	Christopher D. Manning},
	title     = {Effective approaches to attention-based neural machine translation},
	booktitle = {Proceedings of the 2015 Conference on Empirical Methods in Natural Language Processing},
	pages     = {1412--1421},
	year      = {2015}
}

@inproceedings{Chen2020Neural,
	author    = {Lu Chen and
	Yanbin Zhao and
	Boer Lyu and
	Lesheng Jin and
	Zhi Chen and
	Su Zhu and
	Kai Yu},
	title     = {Neural graph matching networks for {Chinese} short text matching},
	booktitle = {Proceedings of the 58th Annual Meeting of the Association for Computational Linguistics},
	pages     = {6152--6158},
	year      = {2020}
}

@inproceedings{liu2018lcqmc,
	title={{LCQMC}: {A} large-scale {Chinese} question matching corpus},
	author={Liu, Xin and Chen, Qingcai and Deng, Chong and Zeng, Huajun and Chen, Jing and Li, Dongfang and Tang, Buzhou},
	booktitle={Proceedings of the 27th International Conference on Computational Linguistics},
	pages={1952--1962},
	year={2018}
}

@inproceedings{Lai2017RACE,
	author    = {Guokun Lai and
	Qizhe Xie and
	Hanxiao Liu and
	Yiming Yang and
	Eduard H. Hovy},
	title     = {{RACE:} {L}arge-scale reading comprehension dataset From examinations},
	booktitle = {Proceedings of the 2017 Conference on Empirical Methods in Natural	Language Processing},
	pages     = {785--794},
	year      = {2017}
}

@inproceedings{Jawahar2019What,
	author    = {Ganesh Jawahar and
	Beno{\^{\i}}t Sagot and
	Djam{\'{e}} Seddah},
	title     = {What does {BERT} learn about the structure of language?},
	booktitle = {Proceedings of the 57th Conference of the Association for Computational Linguistics},
	pages     = {3651--3657},
	year      = {2019}
}

@inproceedings{Reimers2019Sentence,
	author    = {Nils Reimers and
	Iryna Gurevych},
	title     = {Sentence-BERT: {S}entence embeddings using {S}iamese BERT-networks},
	booktitle = {Proceedings of the 2019 Conference on Empirical Methods in Natural	Language Processing and the 9th International Joint Conference on Natural Language Processing},
	pages     = {3980--3990},
	year      = {2019}
}

@article{Nitish2014Dropout,
	author    = {Nitish Srivastava and Geoffrey E. Hinton and Alex Krizhevsky and Ilya Sutskever and Ruslan Salakhutdinov},
	title     = {Dropout: {A} simple way to prevent neural networks from overfitting},
	journal   = {Journal of Machine Learning Research},
	volume    = {15},
	number    = {1},
	pages     = {1929--1958},
	year      = {2014}
}

@inproceedings{Lu2020Improving,
	author    = {Junyu Lu and
	Xiancong Ren and
	Yazhou Ren and
	Ao Liu and
	Zenglin Xu},
	title     = {Improving Contextual Language Models for Response Retrieval in Multi-Turn
	Conversation},
	booktitle = {Proceedings of the 43rd International {ACM} {SIGIR} Conference on
	Research and Development in Information Retrieval},
	pages     = {1805--1808},
	year      = {2020}
}

@inproceedings{Whang2020Effective,
	author    = {Taesun Whang and
	Dongyub Lee and
	Chanhee Lee and
	Kisu Yang and
	Dongsuk Oh and
	Heuiseok Lim},
	title     = {An Effective Domain Adaptive Post-Training Method for {BERT} in Response
	Selection},
	booktitle = {Proceedings of the 21st Annual Conference of the International Speech Communication Association},
	pages     = {1585--1589},
	year      = {2020}
}

@inproceedings{Houlsby2019Parameter,
	author    = {Neil Houlsby and
	Andrei Giurgiu and
	Stanislaw Jastrzebski and
	Bruna Morrone and
	Quentin de Laroussilhe and
	Andrea Gesmundo and
	Mona Attariyan and
	Sylvain Gelly},
	title     = {Parameter-Efficient Transfer Learning for {NLP}},
	booktitle = {Proceedings of the 36th International Conference on Machine Learning},
	pages     = {2790--2799},
	year      = {2019}
}

@inproceedings{Gu2020Speaker,
	author    = {Jia{-}Chen Gu and
	Tianda Li and
	Quan Liu and
	Zhen{-}Hua Ling and
	Zhiming Su and
	Si Wei and
	Xiaodan Zhu},
	title     = {Speaker-Aware {BERT} for Multi-Turn Response Selection in Retrieval-Based
	Chatbots},
	booktitle = {Proceedings of the 29th {ACM} International Conference on Information
	and Knowledge Management},
	pages     = {2041--2044},
	year      = {2020}
}

@inproceedings{Whang2021Response,
	author    = {Taesun Whang and
	Dongyub Lee and
	Dongsuk Oh and
	Chanhee Lee and
	Kijong Han and
	Dong{-}hun Lee and
	Saebyeok Lee},
	title     = {Do Response Selection Models Really Know What's Next? Utterance Manipulation
	Strategies for Multi-turn Response Selection},
	booktitle = {Proceedings of the 35th {AAAI} Conference on Artificial Intelligence},
	pages     = {14041--14049},
	year      = {2021}
}

@inproceedings{Xu2021Learning,
	author    = {Ruijian Xu and
	Chongyang Tao and
	Daxin Jiang and
	Xueliang Zhao and
	Dongyan Zhao and
	Rui Yan},
	title     = {Learning an Effective Context-Response Matching Model with Self-Supervised
	Tasks for Retrieval-based Dialogues},
	booktitle = {Proceedings of the 35th {AAAI} Conference on Artificial Intelligence},
	pages     = {14158--14166},
	year      = {2021}
}

@article{Pre2019Cui,
  author    = {Yiming Cui and
               Wanxiang Che and
               Ting Liu and
               Bing Qin and
               Ziqing Yang},
  title     = {Pre-Training With Whole Word Masking for Chinese {BERT}},
  journal   = {{IEEE}/{ACM} Transactions on Audio, Speech, and Language Processing},
  volume    = {29},
  pages     = {3504--3514},
  year      = {2021}
}

@article{sun2019ernie,
	title={{ERNIE}: {E}nhanced representation through knowledge integration},
	author={Sun, Yu and Wang, Shuohuan and Li, Yukun and Feng, Shikun and Chen, Xuyi and Zhang, Han and Tian, Xin and Zhu, Danxiang and Tian, Hao and Wu, Hua},
	journal={arXiv preprint arXiv:1904.09223},
	year={2019}
}

@inproceedings{Lyu2021LET,
	author    = {Boer Lyu and
	Lu Chen and
	Su Zhu and
	Kai Yu},
	title     = {{LET:} {L}inguistic knowledge enhanced graph transformer for {C}hinese short text matching},
	booktitle = {Proceedings of the 35th {AAAI} Conference on Artificial Intelligence},
	pages     = {13498--13506},
	year      = {2021}
}

@inproceedings{Liu2020BERT,
	author    = {Weijie Liu and
	Peng Zhou and
	Zhe Zhao and
	Zhiruo Wang and
	Qi Ju and
	Haotang Deng and
	Ping Wang},
	title     = {{K-BERT:} {E}nabling language representation with knowledge graph},
	booktitle = {Proceedings of the 34th {AAAI} Conference on Artificial Intelligence},
	pages     = {2901--2908},
	year      = {2020}
}

@inproceedings{Parikh2018ElimiNet,
	author    = {Soham Parikh and
	Ananya Sai and
	Preksha Nema and
	Mitesh M. Khapra},
	title     = {{ElimiNet}: {A} model for eliminating options for reading comprehension
	with Multiple Choice Questions},
	booktitle = {Proceedings of the 27th International Joint Conference on Artificial Intelligence},
	pages     = {4272--4278},
	year      = {2018}
}

@inproceedings{Chen2019Convolutional,
	author    = {Zhipeng Chen and
	Yiming Cui and
	Wentao Ma and
	Shijin Wang and
	Guoping Hu},
	title     = {Convolutional spatial attention model for reading comprehension with multiple-choice questions},
	booktitle = {Proceedings of the 33rd {AAAI} Conference on Artificial Intelligence},
	pages     = {6276--6283},
	year      = {2019}
}

@article{Xu2017Towards,
	author    = {Yichong Xu and
	Jingjing Liu and
	Jianfeng Gao and
	Yelong Shen and
	Xiaodong Liu},
	title     = {Towards human-level machine reading comprehension: {R}easoning and inference with multiple strategies},
	journal   = {CoRR},
	year      = {2017}
}

@inproceedings{Zhang2020DCMN,
	author    = {Shuailiang Zhang and
	Hai Zhao and
	Yuwei Wu and
	Zhuosheng Zhang and
	Xi Zhou and
	Xiang Zhou},
	title     = {{DCMN+:} {D}ual co-matching network for multi-choice reading comprehension},
	booktitle = {Proceedings of the 34th {AAAI} Conference on Artificial Intelligence},
	pages     = {9563--9570},
	year      = {2020}
}

@inproceedings{Peters2018Deep,
	author    = {Matthew E. Peters and
	Mark Neumann and
	Mohit Iyyer and
	Matt Gardner and
	Christopher Clark and
	Kenton Lee and
	Luke Zettlemoyer},
	title     = {Deep contextualized word representations},
	booktitle = {Proceedings of the 2018 Conference of the North American Chapter of the Association for Computational Linguistics},
	pages     = {2227--2237},
	year      = {2018}
}

@inproceedings{Richardson2020Probing,
	author    = {Kyle Richardson and
	Hai Hu and
	Lawrence S. Moss and
	Ashish Sabharwal},
	title     = {Probing natural language inference models through semantic fragments},
	booktitle = {Proceedings of the Thirty-Fourth {AAAI} Conference on Artificial Intelligence},
	pages     = {8713--8721},
	year      = {2020}
}

@article{Zhang2020Neural,
	author    = {Biao Zhang and
	Deyi Xiong and
	Jun Xie and
	Jinsong Su},
	title     = {Neural machine translation with {GRU}-gated attention model},
	journal   = {{IEEE} Trans. Neural Networks Learn. Syst.},
	volume    = {31},
	number    = {11},
	pages     = {4688--4698},
	year      = {2020}
}

@inproceedings{Liu2020RikiNet,
	author    = {Dayiheng Liu and
	Yeyun Gong and
	Jie Fu and
	Yu Yan and
	Jiusheng Chen and
	Daxin Jiang and
	Jiancheng Lv and
	Nan Duan},
	title     = {RikiNet: {R}eading Wikipedia pages for natural question answering},
	booktitle = {Proceedings of the 58th Annual Meeting of the Association for Computational
	Linguistics},
	pages     = {6762--6771},
	year      = {2020}
}

@inproceedings{Lowe2015Ubuntu,
	author    = {Ryan Lowe and
	Nissan Pow and
	Iulian Serban and
	Joelle Pineau},
	title     = {The {Ubuntu} Dialogue Corpus: {A} Large Dataset for Research in Unstructured
	Multi-Turn Dialogue Systems},
	booktitle = {Proceedings of the 16th Annual Meeting	of the Special Interest Group on Discourse and Dialogue},
	pages     = {285--294},
	year      = {2015}
}

@inproceedings{Wang2017Bilateral,
	author    = {Zhiguo Wang and
	Wael Hamza and
	Radu Florian},
	title     = {Bilateral Multi-Perspective Matching for Natural Language Sentences},
	booktitle = {Proceedings of the 26th International Joint Conference on Artificial Intelligence},
	pages     = {4144--4150},
	year      = {2017}
}



@inproceedings{Zhu20118Hierarchical,
	author    = {Haichao Zhu and
	Furu Wei and
	Bing Qin and
	Ting Liu},
	title     = {Hierarchical Attention Flow for Multiple-Choice Reading Comprehension},
	booktitle = {Proceedings of the 32nd {AAAI} Conference on Artificial Intelligence},
	pages     = {6077--6085},
	year      = {2018}
}

@article{Gilbert2000,
	title = {Interactions between attention, context and learning in primary visual cortex},
	journal = {Vision Research},
	volume = {40},
	number = {10},
	pages = {1217-1226},
	year = {2000},
	author = {Charles Gilbert and Minami Ito and Mitesh Kapadia and Gerald Westheimer}
}

@article{Knoeferle2020,
	title = {How context influences language processing and comprehension},
	journal = {Research Outreach},
	volume = {},
	number = {},
	pages = {DOI: 10.32907/RO-114-170173},
	year = {2020},
	author = {P. Knoeferle}
}

@ARTICLE{Oberauer2019,
	AUTHOR = "K. Oberauer",
	TITLE = "Working memory and attention - {A} conceptual analysis and review",
	JOURNAL = "Journal of Cognition",
	VOLUME = {2},
	NUMBER = {1},
	PAGES = {36},
	MONTH = "",
	YEAR = {2019}
}

@article{Li2021Small,
	author    = {Yuntao Li and
	Can Xu and
	Huang Hu and
	Lei Sha and
	Yan Zhang and
	Daxin Jiang},
	title     = {Small Changes Make Big Differences: {I}mproving Multi-turn Response
	Selection in Dialogue Systems via Fine-Grained Contrastive Learning},
	journal   = {CoRR},
	year      = {2021}
}

@ARTICLE{Willems2021,
	AUTHOR = "R.M. Willems and M.V. Peelen",
	TITLE = "How context changes the neural basis of perception and language",
	JOURNAL = "iScience",
	VOLUME = {24},
	NUMBER = {5},
	PAGES = {102392},
	MONTH = "",
	YEAR = {2021}
}

@inproceedings{Wang2018Matching,
	author    = {Shuohang Wang and
	Mo Yu and
	Jing Jiang and
	Shiyu Chang},
	title     = {A Co-Matching Model for Multi-choice Reading Comprehension},
	booktitle = {Proceedings of the 56th Annual Meeting of the Association for Computational Linguistics},
	pages     = {746--751},
	year      = {2018}
}

@inproceedings{Huang2019Multi,
	author    = {Qiang Huang and
	Jianhui Bu and
	Weijian Xie and
	Shengwen Yang and
	Weijia Wu and
	Liping Liu},
	title     = {Multi-task Sentence Encoding Model for Semantic Retrieval in Question
	Answering Systems},
	booktitle = {Proceedings of the International Joint Conference on Neural Networks},
	pages     = {1--8},
	year      = {2019}
}

@inproceedings{Han2021Fine,
	author    = {Janghoon Han and
	Taesuk Hong and
	Byoungjae Kim and
	Youngjoong Ko and
	Jungyun Seo},
	title     = {Fine-grained Post-training for Improving Retrieval-based Dialogue
	Systems},
	booktitle = {Proceedings of the 2021 Conference of the North American Chapter of
	the Association for Computational Linguistics: {H}uman Language Technologies},
	pages     = {1549--1558},
	year      = {2021}
}

@inproceedings{Wu2017Sequential,
	author    = {Yu Wu and
	Wei Wu and
	Chen Xing and
	Ming Zhou and
	Zhoujun Li},
	title     = {Sequential Matching Network: {A} New Architecture for Multi-turn Response Selection in Retrieval-Based Chatbots},
	booktitle = {Proceedings of the 55th Annual Meeting of the Association for Computational Linguistics},
	pages     = {496--505},
	year      = {2017}
}

@inproceedings{Zhang2018Modeling,
	author    = {Zhuosheng Zhang and
	Jiangtong Li and
	Pengfei Zhu and
	Hai Zhao and
	Gongshen Liu},
	title     = {Modeling Multi-turn Conversation with Deep Utterance Aggregation},
	booktitle = {Proceedings of the 27th International Conference on Computational Linguistics},
	pages     = {3740--3752},
	year      = {2018}
}

@article{Kadlec2015Improved,
	author    = {Rudolf Kadlec and
	Martin Schmid and
	Jan Kleindienst},
	title     = {Improved Deep Learning Baselines for {Ubuntu} Corpus Dialogs},
	journal   = {CoRR},
	volume    = {abs/1510.03753},
	year      = {2015}
}

@inproceedings{Zhou2018Multi,
	author    = {Xiangyang Zhou and
	Lu Li and
	Daxiang Dong and
	Yi Liu and
	Ying Chen and
	Wayne Xin Zhao and
	Dianhai Yu and
	Hua Wu},
	title     = {Multi-Turn Response Selection for Chatbots with Deep Attention Matching
	Network},
	booktitle = {Proceedings of the 56th Annual Meeting of the Association for Computational Linguistics},
	pages     = {1118--1127},
	year      = {2018}
}

@inproceedings{Tao2019One,
	author    = {Chongyang Tao and
	Wei Wu and
	Can Xu and
	Wenpeng Hu and
	Dongyan Zhao and
	Rui Yan},
	title     = {One Time of Interaction May Not Be Enough: {G}o Deep with an Interaction-over-Interaction
	Network for Response Selection in Dialogues},
	booktitle = {Proceedings of the 57th Conference of the Association for Computational Linguistics},
	pages     = {1--11},
	year      = {2019}
}

@article{Chen2019Sequential,
	author    = {Qian Chen and
	Wen Wang},
	title     = {Sequential Attention-based Network for Noetic End-to-End Response
	Selection},
	journal   = {CoRR},
	volume    = {abs/1901.02609},
	year      = {2019}
}

@inproceedings{chen2017enhanced,
  title={Enhanced {LSTM} for Natural Language Inference},
  author={Chen, Qian and Zhu, Xiaodan and Ling, Zhen-Hua and Wei, Si and Jiang, Hui and Inkpen, Diana},
  booktitle={Proceedings of the 55th Annual Meeting of the Association for Computational Linguistics},
  pages={1657--1668},
  year={2017}
}


@inproceedings{Yuan2019Multi,
	author    = {Chunyuan Yuan and
	Wei Zhou and
	Mingming Li and
	Shangwen Lv and
	Fuqing Zhu and
	Jizhong Han and
	Songlin Hu},
	title     = {Multi-hop Selector Network for Multi-turn Response Selection in Retrieval-based
	Chatbots},
	booktitle = {Proceedings of the 2019 Conference on Empirical Methods in Natural
	Language Processing and the 9th International Joint Conference on
	Natural Language Processing},
	pages     = {111--120},
	year      = {2019}
}


@inproceedings{zeng2021cr,
  title={{CR-Fill: G}enerative image inpainting with auxiliary contextual reconstruction},
  author={Zeng, Yu and Lin, Zhe and Lu, Huchuan and Patel, Vishal M},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  pages={14164--14173},
  year={2021}
}

@article{xiang2022deep,
  title={Deep Learning for Image Inpainting: {A} Survey},
  author={Xiang, Hanyu and Zou, Qin and Nawaz, Muhammad Ali and Huang, Xianfeng and Zhang, Fan and Yu, Hongkai},
  journal={Pattern Recognition},
  pages={109046},
  year={2022}
}

@article{liu2022deep,
  title={Deep Image Inpainting with Enhanced Normalization and Contextual Attention},
  author={Liu, Jialu and Gong, Maoguo and Tang, Zedong and Qin, AK and Li, Hao and Jiang, Fenlong},
  journal={IEEE Transactions on Circuits and Systems for Video Technology},
  year={2022}
}

@article{song2022contextual,
  title={Contextual Attention Network for Emotional Video Captioning},
  author={Song, Peipei and Guo, Dan and Cheng, Jun and Wang, Meng},
  journal={IEEE Transactions on Multimedia},
  year={2022},
  publisher={IEEE}
}

@inproceedings{zhang2022word,
  title={Word Sense Disambiguation with Knowledge-Enhanced and Local Self-Attention-based Extractive Sense Comprehension},
  author={Zhang, Guobiao and Lu, Wenpeng and Peng, Xuepeng and Wang, Shoujin and Kan, Baoshuo and Yu, Rui},
  booktitle={Proceedings of the 29th International Conference on Computational Linguistics},
  year={2022}
}

@inproceedings{zhang2021self,
  title={Self-supervised bilingual syntactic alignment for neural machine translation},
  author={Tianfu Zhang and Heyan Huang and Longbing Cao and Chong Feng},
  booktitle={Proceedings of the 35th AAAI Conference on Artificial Intelligence},
  pages={14454--14462},
  year={2021}
}
